A Parametric Class of Approximate Gradient Updates for Policy Optimization

Approaches to policy optimization have been motivated from diverse principles, based on how the parametric model is interpreted (e.g. value versus policy representation) or how the learning objective is formulated, yet they share a common goal of maximizing expected return. To better capture the commonalities and identify key differences between policy optimization methods, we develop a unified perspective that re-expresses the underlying updates in terms of a limited choice of gradient form and scaling function. In particular, we identify a parameterized space of approximate gradient updates for policy optimization that is highly structured, yet covers both classical and recent examples, including PPO. As a result, we obtain novel yet well motivated updates that generalize existing algorithms in a way that can deliver benefits both in terms of convergence speed and final result quality. An experimental investigation demonstrates that the additional degrees of freedom provided in the parameterized family of updates can be leveraged to obtain non-trivial improvements both in synthetic domains and on popular deep RL benchmarks.

==> sections/gradients.tex <==
%!TEX root = ../main.tex

\section{Connection Between Various Objective Gradients}\label{sec:unification}
\subsection{Target Estimates}
All methods implicitly or explicitly have some form of estimating a target discounted return. This could be max at next state for DQN or the Monte-Carlo estimate for PG or Td-lambda version.

In this section, we derive sample estimates for the gradients of four different objectives grounded under the set of common assumptions from Section \ref{sec:setting}. For simplicity, we only consider the on-policy expressions in this Section, which will be extended to the offline scenario in Section \ref{sec:scaling}.
\subsection{Q-learning Gradient}\label{sec:q}
We first consider the squared error minimization objective for $Q-$learning, which fits a parameterized $q_\theta(s, a)$ to the target return, $\hat{T}(s, a)$ on a dataset $\mathcal{D}$.
Note that both $\mathcal{D}$ as well as the target sample, $\hat{T}(s, a)$ may implicitly even depend on the policy $\pi$, but these dependencies are 
never considered for the gradient calculation while minimizing the squared prediction error in $Q-$learning.
Under the assumptions from Section \ref{sec:setting}, we can write the gradient of the negative MSE objective as:
\begin{align}
	G_{QL} &= - \nabla_\theta \frac{1}{2} \expectation_{(s, a) \sim \mathcal{D}} \left[ ( \hat{T}(s, a) -  q_\theta(s, a) )^2 \right] \\
	       &= \expectation_{(s, a) \sim \mathcal{D}} (\hat{T}(s, a) - q_\theta(s, a)) \nabla_\theta q_\theta(s, a) \\
	       &= \expectation_{(s, a) \sim D_\pi} \left[ (Q^\pi(s, a) - q_\theta(s, a)) \nabla_\theta q_\theta(s, a)\right] \text{ using Equation \ref{eqn:onpolicy} and assuming $\hat{T} \equiv Q^\pi$ }
\end{align}
Written as a single sample stochastic gradient estimate of the maximization objective, we have:
\begin{align}
	G_{QL} &= \expectation_{(s, a) \sim D_\pi} \hat{G}_{QL}(s, a) \\
	\mbox{ where, }~~~ \hat{G}_{QL}(s, a, \theta) &\triangleq \left(Q^\pi(s, a) - q_\theta(s, a) \right) \nabla_\theta q_\theta(s, a) \label{eqn:ql}
\end{align}
% \begin{equation}\label{eqn:ql}
% 	\hat{G}_{QL}(s, a, \theta) \triangleq \left(Q^\pi(s, a) - q_\theta(s, a) \right) \nabla_\theta q_\theta(s, a)
% \end{equation}

\subsection{Policy Gradient with Policy Baseline (PGPB)}\label{sec:pg}
From the standard policy gradient theorem \citep{pgoriginal}:
\begin{align}
	G_{PG}(\theta) &= \sum_s d^\pi_\mu(s) \sum_a Q^\pi(s, a) \nabla_\theta \pi_\theta(a | s) \\
		       &= \sum_s d^\pi_\mu(s) \sum_a \pi_\theta(a | s) Q^\pi(s, a) \nabla_\theta \log{\pi_\theta(a | s)} \\
		       &= \expectation_{(s, a) \sim D_\pi } \left[ Q^\pi(s, a) \nabla_\theta  \log{\pi_\theta(a | s)} \right] \label{eqn:exact_pg}
\end{align}
To derive an unbiased sample estimate for Equation \ref{eqn:exact_pg}, there are several versions corresponding to particular choices of control variates, also commonly referred to as baselines. 
In order to relate to the $Q-$learning gradients, consider a state-action baseline equal to the policy logits themselves, i.e. $q_\theta(s, a)$. Note that Assumption \ref{assumption:softmax} implies the following identity:
\begin{equation}\label{eqn:softmax_grad}
\nabla_\theta \log{\pi_\theta(a|s)} = \nabla_\theta q_\theta(s, a) - \sum_u \pi_\theta(u|s) \nabla_\theta q_\theta(s, u)
\end{equation}
Using this, we can write\footnote{We suppress $\pi$'s dependence on $\theta$ when there are no gradients through that term.}:
\begin{align}
	&G_{PG}(\theta) = \expectation_{(s, a) \sim D_\pi} \left[ Q^\pi(s, a) \nabla_\theta \log{\pi_\theta(a|s)} \right] \\
		       &= \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a|s \sim \pi} \left[ (Q^\pi(s, a) - q_\theta(s, a))\nabla_\theta \log{\pi_\theta(a|s)}  \right] 
		       + \expectation_{u | s \sim \pi} \left[ q_\theta(s, u) \nabla_\theta \log{\pi_\theta(u|s)} \right] \right]\\
		       &= \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a | s \sim \pi} \left[ (Q^\pi(s, a) - q_\theta(s, a))\nabla_\theta \log{\pi_\theta(a|s)}  \right] 
		       + \nabla_\theta \expectation_{u|s \sim \pi_\theta} \left[ \hat{q}_\theta(s, u) \right] \right]\\ \label{eqn:hat}
		       &= \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a|s \sim \pi} \left[ \Big(Q^\pi(s, a) - q_\theta(s, a)\Big)\Big(\nabla_\theta q_\theta(s, a) - \expectation_{u|s \sim \pi} \left[ \nabla_\theta q_\theta(s, u) \right]\Big)
\right]  + \nabla_\theta \expectation_{u|s \sim \pi_\theta} \left[ \hat{q}_\theta(s, u) \right] \right]
\end{align}
In the last term in Equation \ref{eqn:hat}, we use $\hat{q}_\theta$ rather than $q_\theta$ to denote a partial derivative that does not consider $\hat{q}_\theta$ for the gradient with respect to $\theta$ (i.e., a `stop gradient').
We can therefore define a sample gradient estimate for $G_{PG}(\theta) = \expectation_{(s, a) \sim D_\pi} \hat{G}_{PGPB}(s, a, \theta)$ as:
\begin{equation}\label{eqn:pgpb}
	\hat{G}_{PGPB}(s, a, \theta) \triangleq  \Big(Q^\pi(s, a) - q_\theta(s, a)\Big)\Big(\nabla_\theta q_\theta(s, a) - \expectation_{u|s \sim \pi} \left[ \nabla_\theta q_\theta(s, u) \right]\Big)
+ \nabla_\theta \expectation_{u|s \sim \pi_\theta} \left[ \hat{q}_\theta(s, u) \right]
\end{equation}
The gradient estimate $\hat{G}_{PGPB}(s, a, \theta)$ is unbiased for the expected reward objective. Notice that there are two terms, $\expectation_{u|s \sim \pi}\left[ \nabla_\theta q_\theta(s, u) \right]$ and  $\nabla_\theta \expectation_{u|s \sim \pi_\theta} \left[ \hat{q}_\theta(s, u) \right]$
in Equation \ref{eqn:pgpb} which do not depend on the sampled action, $a$ or the reward estimate, $Q^\pi(s, a)$. Therefore,
both these terms can be computed easily (with zero variance in case of discrete actions, or low variance with the reparameterization trick in case of continuous actions for suitable parameterization; and without querying the environment or the dataset).
Comparing $\hat{G}_{PGPB}(s, a, \theta)$ with $\hat{G}_{QL}(s, a, \theta)$ from Equation \ref{eqn:ql}, we can interpret the $Q-$learning gradient as a biased version of policy gradient obtained by dropping the two aforementioned terms in Equation \ref{eqn:pgpb}.
\subsection{Variance Minimization Gradient}\label{sec:v}
By contrast, consider an alternate gradient estimate that results from dropping only one of the two additional terms in $\hat{G}_{PGPB}$ compared to $\hat{G}_Q$, $\nabla_\theta \expectation_{u|s \sim \pi_\theta} \left[ \hat{q}_\theta(s, u) \right]$. Denote this by $\hat{G}_{V}$:
\begin{equation}\label{eqn:var}
\hat{G}_{V}(s, a, \theta) \triangleq \Big(Q^\pi(s, a) - q_\theta(s, a)\Big)\Big(\nabla_\theta q_\theta(s, a) - \expectation_{u|s \sim \pi} \left[ \nabla_\theta q_\theta(s, u) \right]\Big)
\end{equation}
As shown below, this is equivalent to the gradient of an objective which minimizes the variance, instead of the expectation of the squared error across actions. 
\begin{align}
	& \expectation \left[\hat{G}_{V}(s, a, \theta)\right] = \expectation_{(s, a) \sim D_\pi}\left[ \Big(Q^\pi(s, a) - q_\theta(s, a)\Big)\Big(\nabla_\theta q_\theta(s, a) - \expectation_{u|s \sim \pi} \left[ \nabla_\theta q_\theta(s, u) \right]\Big)
\right] \\
									 &= \expectation_{s \sim d^{\pi}_\mu} \left[ \expectation_{a|s \sim \pi} \Big[ \Big(Q^\pi(s, a) - q_\theta(s, a)\Big)\nabla_\theta q_\theta(s, a)\Big] - \expectation_{a|s \sim \pi} \Big[Q^\pi(s, a) - q_\theta(s, a) \Big] \expectation_{u|s \sim \pi} \Big[ \nabla_\theta q_\theta(s, u) \Big] \right] \\
									 &= -\frac{1}{2} \expectation_{s \sim d^{\pi}_\mu} \left[ \nabla_\theta \expectation_{a|s \sim \hat{\pi}} \left[ (Q^\pi(s, a) - q_\theta(s, a))^2 \right] - \nabla_\theta \left( \expectation_{a|s \sim \hat{\pi}} \left[Q^\pi(s, a) - q_\theta(s, a)\right]\right)^2 \right] \\
									 &= -\frac{1}{2} \expectation_{s \sim d^{\pi}_\mu} \nabla_\theta \variance_{a|s \sim \hat{\pi}}\Big[Q^\pi(s, a) - q_\theta(s, a) \Big] \mbox{ where } \variance \mbox{denotes variance.}
\end{align}
In the last two equalities above, we use $\hat{\pi}$ rather than $\pi$ to indicate that the gradient operator can pass through the expectations without considering the implicit dependency of $\pi$ on $\theta$.

\subsection{Imitation Learning}\label{sec:il}
Next, consider the log-likelihood objective with respect to a target distribution defined by $\hat{p}_T(a|s) \triangleq \exp{\Big(Q^\pi(s, a) - F(Q^\pi)(s)\Big)}$, where $F(q)(s) \triangleq \log{\sum_{a} \exp{q(s, a)}}$ is used to denote the LogSumExp reduction over actions for an arbitrary state-action value function $q(s, a)$. Below, we derive an expression for the gradient of a Maximum Likelihood objective, which highlights it's differences with respect to the squared error objective of $Q-$learning.
\begin{align}
	G_{IL} &\triangleq \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a|s \sim \hat{p}_T} \nabla_\theta \log{\pi_\theta(a|s)} \right] \\
	       &= \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a|s \sim \hat{p}_T} \left[ \nabla_\theta q_\theta(s, a) - \sum_u \pi_\theta(u|s) \nabla_\theta q_\theta(s, u) \right] \right] \\
	       &= \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a|s \sim \hat{p}_T} \Big[ \nabla_\theta q_\theta(s, a) \Big] - \sum_u \pi_\theta(u|s) \nabla_\theta q_\theta(s, u) \right] \\
	       &= \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a|s \sim \pi} \left[ \frac{\hat{p}_T(a|s)}{\pi_\theta(a|s)} \nabla_\theta q_\theta(s, a) \right] - \expectation_{u|s \sim \pi} \Big[ \nabla_\theta q_\theta(s, u) \Big] \right] \\
	       &= \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a|s \sim \pi} \left[ \left(\frac{\hat{p}_T(a|s)}{\pi_\theta(a|s)} - 1\right) \nabla_\theta q_\theta(s, a) \right] \right] \\
	       % &= \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a|s \sim \pi} \left[ \left(e^{Q^\pi(s, a) - q_\theta(s, a) + F(q_\theta)(s) - F(Q^\pi)(s)} - 1\right) \nabla_\theta q_\theta(s, a) \right] \right]  \\
	       &= \expectation_{s \sim d^\pi_\mu} \left[ \expectation_{a|s \sim \pi} \left[ \left(\exp{\Big(Q^\pi(s, a) - q_\theta(s, a) + F(q_\theta)(s) - F(Q^\pi)(s)\Big)} - 1\right) \nabla_\theta q_\theta(s, a) \right] \right] 
\end{align}
Now consider a biased gradient estimate which drops the log-normalizer difference term, $F(Q^\pi)(s) - F(q_\theta)(s)$, as $\hat{G}_{IL}$.
\begin{equation}\label{eqn:ilo}
	\hat{G}_{IL}(s, a, \theta) \triangleq \Big(\exp\big(Q^\pi(s, a) - q_\theta(s, a)\big) - 1 \Big) \nabla_\theta q_\theta(s, a)
\end{equation}

In \citet{sil}, the authors propose a novel objective derived from modifying $Q-$learning by clipping the prediction error below at 0, which is referred to as self imitation learning.
We write the gradient expression corresponding to the self imitation learning objective as $\hat{G}_{SIL}$ next.
\begin{equation}\label{eqn:silo}
	\hat{G}_{SIL}(s, a, \theta) =  \max(Q^\pi(s, a) - q_\theta(s, a), 0) \nabla_\theta q_\theta(s, a)
\end{equation}
This suggests that an alternate way to interpret the SIL gradient is by considering $\max (x, 0)$ as an approximation to $e^x - 1$. 

\section{Gradient Scaling Functions with Off-Policy Correction}\label{sec:scaling}
Until now, we made an assumption that the sampling distribution for states and actions matches the policy $\pi_\theta$. In this section, that assumption is relaxed. Let $\pi_b$ denote a behavior policy that is different from the current policy. Note that $\pi_b$ may not be explicitly available, but can be estimated using conditional maximum-likelihood as:
\begin{equation}
b = \arg \max_\theta \sum_{(s, a) \sim \mathcal{D} } \log \pi_\theta(a|s)
\end{equation}
Consider off-policy importance weights for action conditionals\footnote{We consider exploration issues outside the scope of
this work and ignore any mismatch in the state-marginals while computing the importance weights.} between the behavior policy and the current policy, $\frac{\pi_\theta(a|s)}{\pi_b(a|s)}$.
To simplify the expressions, denote the off-policy log density ratio and the prediction error as the following two sample dependent scalar `learning signals':
\begin{equation}\label{eq:DeltaO} \Delta_O \triangleq \log
\frac{\pi_\theta(a|s)}{\pi_b(a|s)} \end{equation}
\begin{equation}\label{eq:DeltaR} \Delta_R \triangleq Q^\pi(s, a) - q_\theta(s, a) \end{equation} 
$\Delta_O$ is the logarithm of the off-policy importance weight ratio, and can also be viewed as 
a single sample unbiased estimate of the KL divergence between the behavior and current policies. When the dataset
is on-policy, this implies $\Delta_O = 0$ for all samples, $(s, a)$.
By contrast, $\Delta_R = 0$ when the value prediction error is zero at the current sample, $(s, a)$.
With this notation, the five gradient expressions in Equations \ref{eqn:ql}, \ref{eqn:pgpb}, \ref{eqn:var}, 
\ref{eqn:ilo}, \ref{eqn:silo} can be extended to the off-policy case where the dependence on $\Delta_O$ and $\Delta_R$ can be captured as a function $f: \mathbb{R}^2 \mapsto \mathbb{R}$. 
\begin{align}
	\hat{G}_{QL}(s, a, \theta) &= f_{SQ}(\Delta_O, \Delta_R) \Big( \nabla_\theta q_\theta(s, a) \Big) \label{eqn:q} \\
	\hat{G}_{IL}(s, a, \theta) &= f_{IL}(\Delta_O, \Delta_R)\Big( \nabla_\theta q_\theta(s, a) \Big) \label{eqn:il} \\
	\hat{G}_{SIL}(s, a, \theta) &= f_{SIL}(\Delta_O, \Delta_R)\Big( \nabla_\theta q_\theta(s, a) \Big) \label{eqn:sil} \\
	\hat{G}_{PGPB}(s, a, \theta) &=  f_{SQ}(\Delta_O, \Delta_R)\Big(\nabla_\theta q_\theta(s, a) - \expectation_{u|s \sim \pi} \left[ \nabla_\theta q_\theta(s, u) \right]\Big)
	+ \nabla_\theta \expectation_{u|s \sim \pi_\theta} \left[ \hat{q}_\theta(s, u) \right]  \label{eqn:pg} \\
	\hat{G}_{V}(s, a, \theta) &= f_{SQ}(\Delta_O, \Delta_R)  \Big(\nabla_\theta q_\theta(s, a) - \expectation_{u|s \sim \pi} \left[ \nabla_\theta q_\theta(s, u) \right]\Big) \label{eqn:v} 
\end{align}
The scaling functions, $f_{SQ}, f_{IL}, f_{SIL}$ used above are:
\begin{align}
	f_{SQ}(\Delta_O, \Delta_R) &= e^{\Delta_O}  \Delta_R\\ 
	f_{IL}(\Delta_O, \Delta_R) &= e^{\Delta_O} ( e^{\Delta_R} - 1) \\ 
	f_{SIL}(\Delta_O, \Delta_R)  &= e^{\Delta_O} \max(\Delta_R, 0)
\end{align}
In all cases above, it is easy to verify that $f \in \{f_{SQ}, f_{IL}, f_{SIL}\}$ satisfies the properties listed below. 
While we do not currently have a formal theoretical justification for why these properties might be important, they seem like reasonable constraints to use in constructing closely related, but slightly more general and improved alternative update rules.
\begin{assumption}\label{assumption:constraints}
	Let $f: \mathbb{R}^2 \mapsto \mathbb{R}$ denote a function that captures the dependence of a gradient update on $\Delta_O, \Delta_R$. Then, we require that $f$ satisfies the following constraints:

\begin{enumerate}
	\item $f(\Delta_O, 0) = 0, ~~\forall ~~ \Delta_O \in \mathbb{R}$.
	\item $f(-\infty, \Delta_R) = 0, ~~ \forall ~~ \Delta_R \in \mathbb{R}$. 
	\item $f(\Delta_O, \Delta_R)$ is non-decreasing and convex in $\Delta_R$ for any fixed $\Delta_O$.
	\item $|f(\Delta_O, \Delta_R)|$ is non-decreasing and convex in $\Delta_O$ for any fixed $\Delta_R$. (~$|.|$ denotes absolute value.)
\end{enumerate}
\end{assumption}

\subsection{A practical approximation to the imitation learning gradient}\label{sec:approx}
We now construct a piece-wise polynomial second order approximation\footnote{ILA is used as an abbreviation for `Imitation Learning Approximation'.}, $f_{ILA}$, to $f_{IL}(\Delta_O, \Delta_R) = e^{\Delta_O} (e^{\Delta_R}-1)$ used
in $\hat{G}_{IL}$ from Equation \ref{eqn:il} that is consistent with the 4 constraints listed in Assumption \ref{assumption:constraints}.
\begin{equation}\label{eqn:ila}
	f_{ILA}(\Delta_O, \Delta_R)= 
	\begin{cases}
		-\frac{1}{2}(1 + \Delta_O)^2 , & \text{if } 1 + \Delta_O + \Delta_R \le 0 < 1 + \Delta_O \\
		\Delta_R \max \left(1 + \Delta_O + \frac{\Delta_R}{2}, 0\right) ,              & \text{otherwise}
	\end{cases}
\end{equation}
Using this, we define the approximate gradient estimate $\hat{G}_{ILA}$ as:
\begin{equation}\label{eqn:gila}
\hat{G}_{ILA}(s, a, \theta) = f_{ILA}(\Delta_O, \Delta_R)\Big( \nabla_\theta q_\theta(s, a) \Big) 
\end{equation}
A visualization for the projection of $f_{ILA}$ along various slices of $\Delta_O$ and $\Delta_R$ is shown in Figures ~\ref{fig:slice_r} and \ref{fig:slice_o}. 
When highly off-policy ($\Delta_O \ll 0$), note that $f_{ILA}(\Delta_O, \Delta_R) = 0$ for $\Delta_R$ less than a positive threshold. This threshold increases as the sample becomes more off-policy (ie. as $\Delta_O \rightarrow -\infty$). For large values of $\Delta_R$, the update strength is quadratic in $\Delta_R$. Conversely, it saturates to a small non-positive constant as $\Delta_R \rightarrow -\infty$. 
\begin{figure}
	\centering
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=.9\linewidth]{slice_r}
		\caption{Projection of $f_{ILA}$ onto $\Delta_R$ for varying $\Delta_O$}
		\label{fig:slice_r}
	\end{subfigure}%
	\begin{subfigure}{.5\textwidth}
		\centering
		\includegraphics[width=.9\linewidth]{slice_o}
		\caption{Projection of $f_{ILA}$ onto $\Delta_O$ for varying $\Delta_R$}
		\label{fig:slice_o}
	\end{subfigure}
	\caption{One-dimensional projections for $f_{ILA}(\Delta_O, \Delta_R)$ from Equation \ref{eqn:ila}.}
	\label{fig:test}
\end{figure}

The full range of gradients characterized are summarized in Table~\ref{tab:table1}, which mixes the three types of updates (squared error minimization, variance minimzation and PGPB), with various scaling functions across the rows.  In addition to the six types of updates derived in Equations \ref{eqn:q}, \ref{eqn:il}, \ref{eqn:sil}, \ref{eqn:pg},
\ref{eqn:v}, \ref{eqn:gila}, the table also lists six natural additional variations for a total of twelve update rules being
considered in the numerical evaluations in Section \ref{sec:eval}.
\begin{table}[!ht]
\begin{center}
\caption{A summary of the various gradients derived and their relationships.}
	\renewcommand{\arraystretch}{1.5}
\label{tab:table1}
	\begin{tabular}{|c|c|c|c|} 
		\hline
		\multicolumn{4}{|l|}{$\mathcal{U}_{Q}(f) \equiv f(\Delta_O,\Delta_R)\Big( \nabla_\theta q_\theta(s, a) \Big)$} \\
		\multicolumn{4}{|l|}{$\mathcal{U}_{V}(f) \equiv f(\Delta_O,\Delta_R) \Big(\nabla_\theta q_\theta(s, a) - \expectation_{u|s \sim \pi} \left[ \nabla_\theta q_\theta(s, u) \right]\Big)$ }\\
		\multicolumn{4}{|l|}{$\mathcal{U}_{P}(f) \equiv f(\Delta_O,\Delta_R) \Big(\nabla_\theta q_\theta(s, a) - \expectation_{u|s \sim \pi} \left[ \nabla_\theta q_\theta(s, u) \right]\Big) + \nabla_\theta \expectation_{u|s \sim \pi_\theta} \left[ \hat{q}_\theta(s, u) \right]$} \\
		\hline
		\hline
		$f$ & $\mathcal{U}_Q(f)$ & $\mathcal{U}_V(f)$ & $\mathcal{U}_P(f)$\\
		\hline
		$f_{SQ}(x, y) \triangleq e^x y$ & $\hat{G}_{Q}$& $\hat{G}_{V}$& $\hat{G}_{PGPB}$ \\
		\hline
		$f_{IL}(x, y) \triangleq e^x (e^y - 1) $ & $\hat{G}_{IL}$ & $\hat{G}_{IL, V}$ & $\hat{G}_{IL, PGPB}$ \\
		\hline
		$f_{SIL}(x, y) \triangleq e^{x} \max \left(y, 0\right)$ & $\hat{G}_{SIL}$ & $\hat{G}_{SIL, V}$ & $\hat{G}_{SIL, PGPB}$ \\
		\hline
		$f_{ILA}(x, y) \triangleq 
		 \begin{cases}
			-\frac{1}{2}(1 + x)^2 , & \text{if }1 + x + y \le 0 < 1 + x \\
		y \max \left(1 + x + \frac{y}{2}, 0\right) ,              & \text{otherwise}
	\end{cases}$ & $\hat{G}_{ILA}$ & $\hat{G}_{ILA, V}$ & $\hat{G}_{ILA, PGPB}$\\
		\hline
 \end{tabular}
\end{center}
\end{table}


==> sections/ml.tex <==
%!TEX root = ../main.tex

In this section, we consider an objective inspired by forming the max-likelihood loss to a target distribution and show that this can be approximated as a variation on the scale component. 

\subsection{$f_{MLA}$: A numerically stable approximation}

\subsection{MLA-PPO updates}



==> sections/ppo.tex <==
\textbf{Derive the PPO clipping as a scale component variation}

